Neural Network based End-to-End Query by Example Spoken Term Detection

This paper focuses on the problem of query by example spoken term detection (QbE-STD) in zero-resource scenario. State-of-the-art approaches primarily rely on dynamic time warping (DTW) based template matching techniques using phone posterior or bottleneck features extracted from a deep neural network (DNN). We use both monolingual and multilingual bottleneck features, and show that multilingual features perform increasingly better with more training languages. Previously, it has been shown that the DTW based matching can be replaced with a CNN based matching while using posterior features. Here, we show that the CNN based matching outperforms DTW based matching using bottleneck features as well. In this case, the feature extraction and pattern matching stages of our QbE-STD system are optimized independently of each other. We propose to integrate these two stages in a fully neural network based end-to-end learning framework to enable joint optimization of those two stages simultaneously. The proposed approaches are evaluated on two challenging multilingual datasets: Spoken Web Search 2013 and Query by Example Search on Speech Task 2014, demonstrating in each case significant improvements.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> input/representation_learning_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Representation Learning}\label{sec:rep-learn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this section, we present several FFN architectures to obtain mono-lingual as well as multi-lingual bottleneck features. 
Feed forward networks have been traditionally used to obtain bottleneck features for speech related tasks~\citep{yu2011improved, vesely2012language, szoke2015copingwith}. %Here, we describe the different architectures employed in this study as shown in Figure~\ref{fig:ffn}: 
In this section, we present several FFN architectures to obtain mono-lingual as well as multi-lingual bottleneck features. 


%For this purpose, we train several feed forward networks (FFN) for phone classification using five languages to estimate five distinct monolingual bottleneck features. We also train multilingual FFNs using multitask learning principle~\citep{caruana1997multitask} in order to obtain language independent features. We used a combination of three and five languages to analyze the effect of increasing the language variation for training. The performance of these features are compared using DTW based template matching (Section~\ref{sec:dtw-match}) and the best performing features are used to train a CNN based matching system to replace the DTW.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mono-lingual Neural Network}\label{sec:mono-nn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We train several feed forward networks (FFN) for phone classification using five languages to estimate five distinct monolingual bottleneck features. Our monolingual FFN architecture, consists of 3 fully connected layers of 1024 neurons each, followed by a linear bottleneck layer of 32 neurons, and a fully connected layer of 1024 neurons. The final layer feeds to the output layer of size $c_i$ corresponding to number of classes (e.g. phones) of the $i$-th language. The architecture is presented in Figure~\ref{fig:ffn}.

\begin{figure}
 \centering
 \centerline{\includegraphics[scale=0.6]{./Figure/ffn.png}}
 \label{fig:ffn}
 \caption{Multi-lingual neural network architecture for extracting bottleneck features using 5 different languages. The arrows indicate weight matrices.}
\end{figure}

These monolingual bottleneck features have previously been shown to provide good performance for this task~\citep{szoke2015copingwith}. Here, we reproduce those results and improve on it by training multilingual networks and using the corresponding bottleneck features.

%We have trained one network for each language. The network is a 5 layer fully connected feed forward, the third layer is the linear bottleneck. We have used 5 languages from the GlobalPhone dataset (see Section~\ref{sec:dataset-gp}) to train these networks and used the network to extract bottleneck features to perform QbE-STD experiments. These features have previously been shown to provide good performance for this task~\citep{szoke2015copingwith}. Here, we reproduce those results and improve on it by training multi-lingual network and using the corresponding bottleneck features. 

%The architecture consists of 3 fully connected layer having 1024 neurons each. It is followed by a linear bottleneck layer of 32 neurons. Then we have another fully connected layer of 1024 neurons which feeds to the output layer with corresponding number of classes. 

%\begin{figure}
% \centering
% \begin{minipage}{0.39\textwidth}
%  \centering
%  \centerline{\includegraphics[scale=0.35]{./Figure/1lang_network.png}}
%  \centerline{(a) Mono-lingual Network}
%  \label{fig:1lang-nn}
% \end{minipage}
% \begin{minipage}{0.6\textwidth}
%  \centering
%  \centerline{\includegraphics[scale=0.35]{./Figure/3lang_network.png}}
%  \centerline{(b) Multi-lingual Network for 3 languages}
%  \label{fig:3lang-nn}
%  \end{minipage}
% \caption{Neural network architecture for extracting bottleneck features for mono-lingual as well as multi-lingual network. The arrows indicate weight matrices.}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-lingual Neural Network}\label{sec:multi-nn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Multi-lingual bottleneck features have been studied in the context of ASR in order to obtain language independent representation of speech signal. The multi-lingual networks are designed to have a language independent part and a language dependent part. The language independent part is the first few layers of the network which are shared by all languages. This shared component forces the network to learn language independent characteristics which are shared by the languages for training. On the other hand, the last layers are not shared, enabling the network to learn language dependent components as well. 

In this work, we train 2 different multi-lingual networks using 3 languages and 5 languages in order to analyze the effect of training with additional languages. These networks have different architectures as described in the following:

\begin{itemize}
\item{\bf 3 language Neural Network:} 
The architecture consists of 4 fully connected layer having 1024 neurons each. It is followed by a linear bottleneck layer of 32 neurons. Then we have another fully connected layer of 1024 neurons which feeds to 3 different output layers  corresponding to Portuguese, Spanish and Russian.
\item{\bf 5 language Neural Network:} 
In this case, we have 5 fully connected layer having 1024 neurons each. The extra layer is intended to capture the additional information presented by 2 new languages. Similar to 3 language network, the first 5 layers are followed by a linear bottleneck layer of 32 neurons which feeds to a fully connected layer of 1024 neurons. This layer is connected to 5 different output layers  corresponding to French, German, Portuguese, Spanish and Russian.
\end{itemize}

All neural networks discussed in this section have rectifier linear unit (ReLU) as non-linearity used after each linear transform except in the bottleneck layer and the output layer. The output layer has multiple softmax layers corresponding to each language. 

%\begin{figure}
% \centering
% \centerline{\includegraphics[scale=0.35]{./Figure/5lang_network.png}}
% \label{fig:5lang-nn}
% \caption{Multi-lingual neural network architecture for extracting bottleneck features using 5 different languages. The arrows indicate weight matrices.}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{DTW based Template Matching}\label{sec:dtw-match}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We use different types of bottleneck features (mono and multi lingual) discussed in previous section to perform DTW based template matching for QbE-STD. We follow the system described in Section~\ref{sec:baseline} for this purpose. The only difference is that, instead of using logarithm of cosine distance to construct the distance matrix for DTW, we use cosine distance which has been shown to yield better performance with bottleneck features~\citep{szoke2015copingwith} and our preliminary experiments show similar trend. This query matching can also be performed using CNN as discussed in the following section.
